Measuring Vacancies: Firm-level Evidence from Two Measures

Using firm-level survey- and register-data for both Sweden and Denmark we show systematic mis-measurement in both vacancy measures. While the register-based measure on the aggregate constitutes a quarter of the survey-based measure, the latter is not a super-set of the former. To obtain the full set of unique vacancies in these two databases, the number of survey vacancies should be multiplied by approximately 1.2. Importantly, this adjustment factor varies over time and across firm characteristics. Our findings have implications for both the search-matching literature and policy analysis based on vacancy measures: Observed changes in vacancies can be an outcome of changes in mis-measurement, and are not necessarily changes in the actual number of vacancies.

==> tab_reg_DEN.tex <==
                    &        0.15\sym{***}&        0.33\sym{***}\\
                    &      (0.04)         &      (0.06)         \\\\
                    &        0.01\sym{**} &        0.10\sym{*}  \\
                    &      (0.00)         &      (0.04)         \\
                    &        0.04\sym{***}&        0.20\sym{***}\\
                    &      (0.01)         &      (0.06)         \\
                    &        0.02\sym{***}&        0.06\sym{***}\\
                    &      (0.01)         &      (0.01)         \\
                    &        0.02\sym{***}&        0.27\sym{***}\\
                    &      (0.01)         &      (0.07)         \\
                    &        0.04         &        1.32\sym{**} \\
                    &      (0.03)         &      (0.63)         \\
                    &        0.07         &        1.22\sym{**} \\
                    &      (0.06)         &      (0.49)         \\
                    &        0.04\sym{***}&        0.29\sym{***}\\
                    &      (0.01)         &      (0.08)         \\
                    &        0.27\sym{***}&        0.36\sym{***}\\
                    &      (0.08)         &      (0.09)         \\\\
                    &        0.08\sym{***}&        0.16\sym{***}\\
                    &      (0.01)         &      (0.00)         \\
                    &        0.08\sym{*}  &        1.24\sym{*}  \\
                    &      (0.05)         &      (0.61)         \\
                    &        0.17\sym{**} &        0.76\sym{**} \\
                    &      (0.07)         &      (0.37)         \\
                    &        0.15\sym{***}&        0.33\sym{***}\\
                    &      (0.04)         &      (0.07)         \\\\
                    &        0.28\sym{***}&        0.33\sym{***}\\
                    &      (0.08)         &      (0.08)         \\
                    &        0.19\sym{*}  &        0.66\sym{**} \\
                    &      (0.11)         &      (0.31)         \\
                    &        0.07\sym{***}&        0.38\sym{***}\\
                    &      (0.02)         &      (0.10)         \\
                    &        0.02\sym{***}&        0.14\sym{***}\\
                    &      (0.00)         &      (0.03)         \\


==> tab_regressions_SWE.tex <==
& All                                    & 0.06\sym{***} & 0.13\sym{***}\\
&                                        & (0.01)        & (0.01)         \\
\multicolumn{4}{l}{\emph{By industry}}\\
& Farming, fishery and mining            & 0.21\sym{**}  & 0.73\sym{***}\\
&                                        & (0.10)        & (0.22)         \\
& Manufacturing                          & 0.06\sym{***} & 0.15\sym{***}\\
&                                        & (0.01)        & (0.02)         \\
& Energy and water supply                & 0.01\sym{*}   & 0.08\sym{***}\\
&                                        & (0.01)        & (0.02)         \\
& Construction                           & 0.03\sym{***} & 0.28\sym{***}\\
&                                        & (0.01)        & (0.06)         \\
& Trade, Hotel and Restaurants           & 0.07\sym{***} & 0.16\sym{***}\\
&                                        & (0.01)        & (0.03)         \\
& Transportation, mail and telecom       & 0.05\sym{***} & 0.17\sym{***}\\
&                                        & (0.02)        & (0.04)         \\
& Finance and business services          & 0.07\sym{***} & 0.15\sym{***}\\
&                                        & (0.01)        & (0.02)         \\
& Public services and  personal services & 0.06\sym{***} & 0.09\sym{***}\\
&                                        & (0.01)        & (0.02)         \\
\multicolumn{4}{l}{\emph{By firm size }}\\
& 0-5                                    & 0.06\sym{***} & 0.63\sym{***}\\
&                                        & (0.01)        & (0.15)         \\
& 6-10                                   & 0.16\sym{**}  & 0.46\sym{**} \\
&                                        & (0.08)        & (0.22)         \\
& 11-50                                  & 0.09\sym{***} & 0.25\sym{***}\\
&                                        & (0.01)        & (0.04)         \\
& 50+                                    & 0.06\sym{***} & 0.12\sym{***}\\
&                                        & (0.01)        & (0.01)         \\
\multicolumn{4}{l}{\emph{By value-added/salary per worker}}\\
& Quartile 1                             & 0.09\sym{***} & 0.16\sym{***}\\
&                                        & (0.02)        & (0.02)         \\
& Quartile 2                             & 0.09\sym{***} & 0.16\sym{***}\\
&                                        & (0.01)        & (0.03)         \\
& Quartile 3                             & 0.05\sym{***} & 0.13\sym{***}\\
&                                        & (0.01)        & (0.02)         \\
& Quartile 4                             & 0.05\sym{***} & 0.13\sym{***}\\
&                                        & (0.01)        & (0.02)         \\


==> tab_vac_cross_SWE.tex <==
&0 &376,178&30,821&15,390& 7,263&445,962\\
&1 &12,618& 5,498& 3,720& 2,210&30,914\\
&2 & 2,121&   496&   583&   350& 4,956\\
&3 &   889&   172&   140&   134& 1,875\\
\bottomrule
&Tot&393772&37,325&20,119&10,110&\\
